Strong-weak coupling duality in non-abelian gauge theories

This is a general introduction to electric-magnetic duality in non-abelian gauge theories. In chapter I, I review the general ideas which led in the late 70s to the idea of electric/magnetic duality in quantum field theory. In chapters II and III, I focus mainly on N=2 supersymmetric theories. I present the lagrangians and explain in more or less detail the non-renormalization theorems, rigid special geometry, supersymmetric instanton calculus, charge fractionization, the semiclassical theory of monopoles, duality in Maxwell theory and the famous Seiberg-Witten solution. I discuss various physical applications, as electric charge confinement, chiral symmetry breaking or non-trivial superconformal theories in four dimensions. In Section II.3 new material is presented, related to the computation of the eta invariant of certain Dirac operators coupled minimally to non-trivial monopole field configurations. I explain how these invariants can be obtained exactly by a one-loop calculation in a suitable N=2 supersymmetric gauge theory. This is an unexpected application of the holomorphy properties of N=2 supersymmetry, and constitutes a tremendous simplification of the usual computation. An expanded version of these new results will be published soon.

==> a4.tex <==
\input amssym.def \input amssym.tex
\magnification=1200
\overfullrule=0pt
% definition d'espacements a la francaise
\catcode`\@=11
\pretolerance=500   \tolerance=1000  \brokenpenalty=5000
\catcode`\;=\active
\def;{\relax\ifhmode\ifdim\lastskip>\z@
\unskip\fi\kern.2em\fi\string;}
\catcode`\:=\active
\def:{\relax\ifhmode\ifdim\lastskip>\z@\unskip\fi
\penalty\@M\ \fi\string:}
\catcode`\!=\active
\def!{\relax\ifhmode\ifdim\lastskip>\z@
\unskip\fi\kern.2em\fi\string!}
\catcode`\?=\active
\def?{\relax\ifhmode\ifdim\lastskip>\z@
\unskip\fi\kern.2em\fi\string?}
\def\^#1{\if#1i{\accent"5E\i}\else{\accent"5E #1}\fi}
\def\"#1{\if#1i{\accent"7F\i}\else{\accent"7F #1}\fi}
\frenchspacing
%FONTES
%\font\remerfonte=Adobe Linoscript
\font\rmten=cmr10 at 10truept
\font\rmseven=cmr7 at 7truept
\font\bften=cmbx10 at 10truept
\font\itten=cmti10 at 10truept
%\font\dedicassefonte=pksr2.tfm at 40pt
\font\titrefonte=cmu10 at 9pt
\font\nume=cmu10
\font\chapitrefonte=cmu10 at 30 pt%
\font\sectionfonte=cmbx12
\font\gras=cmbx12
\font\avantfonte=cmu10 at 18pt%
\font\grasmathten=cmmib10 
\font\grasmathseven=cmmib7\font\grasmathfive=cmmib5
\newfam\grasmathfam
\textfont\grasmathfam=\grasmathten\scriptfont\grasmathfam=\grasmathseven
\scriptscriptfont\grasmathfam=\grasmathfive
\def\grasmath{\fam\grasmathfam\grasmathten}
\font\grasmathsyten=cmbsy10
\font\grasmathsyseven=cmbsy7\font\grasmathsyfive=cmbsy5
\newfam\grasmathsyfam
\textfont\grasmathsyfam=\grasmathsyten\scriptfont\grasmathsyfam=\grasmathsyseven
\scriptscriptfont\grasmathsyfam=\grasmathsyfive
\def\grasmathsy{\fam\grasmathsyfam\grasmathsyten}
%
\newtoks\hautdroit\newtoks\hautgauche
\newif\ifpagechapitre\pagechapitretrue
\catcode`\@=12
% interlignes, hauteur et largeur de page, etc...
\def\makeheadline{\vbox to 0pt{\vskip -30pt\line{\vbox to 8.5pt{}
\the\headline}\vss}\nointerlineskip}
\hsize=15.5truecm\vsize=23truecm\voffset 1truecm\hoffset .5truecm
\baselineskip=14pt
\abovedisplayskip=14pt plus 3pt minus 9pt
\belowdisplayskip=14pt plus 3pt minus 9pt
\belowdisplayshortskip=8pt plus3pt minus 4pt
\hautdroit={}\hautgauche={}
\footline={\hfil}
\headline={\ifpagechapitre\hfil\else\titrefonte
\ifodd\pageno\the\hautdroit\hfil\folio
\else\folio\hfil\the\hautgauche\fi\fi}
\parskip=5pt plus 1pt minus 1pt
%
\def\tvi{\vrule height 12pt depth 5pt width 0pt}
\def\tv{\tvi\vrule}
\def\tvp{\vrule height 7.7pt depth 3.5pt width 0pt\vrule}
\def\supbul{\vskip 6pt plus 2pt minus 1pt\noindent\null\quad $\bullet$\ }
%
\countdef\parno=100
\countdef\subparno=101
\countdef\chapno=102
\countdef\numo=103
\numo=0
\parno=0
\subparno=1
\chapno=0
\def\numero{\global\advance\numo by 1
\hbox{({\uppercase\expandafter{\romannumeral\the\chapno}}.\the\numo)}}
%
% CHAPITRES ET SECTIONS
%
\def\chapitre#1]#2]{\numo=0\parno=0\subparno=1\advance\chapno by 1
\ifodd\pageno\null\vfill
{\noindent\chapitrefonte
{\uppercase\expandafter{\romannumeral\the\chapno}}\ \ #2}
\hautgauche={{\uppercase\expandafter{\romannumeral\the\chapno}}\ \ #1}
\hautdroit=\hautgauche\pagechapitretrue
\vskip 5cm\null\eject\null\eject\global\pagechapitrefalse
\else\pagechapitretrue\vfill\null\eject 
\null\vfill
{\noindent\chapitrefonte
{\uppercase\expandafter{\romannumeral\the\chapno}}\ \ #2}
\hautgauche={{\uppercase\expandafter{\romannumeral\the\chapno}}\ \ #1}
\hautdroit=\hautgauche\pagechapitretrue
\vskip 5cm\eject\null\eject\global\pagechapitrefalse\fi}
\def\section#1]{\subparno=1\goodbreak\bigskip\bigskip\centerline{
\global\advance\parno by 1\sectionfonte\the\parno .\ \ #1}
\bigskip\nobreak\hautdroit={\the\parno .\ \ #1}}
\def\ssection#1]{\goodbreak\medskip
{\noindent $\triangleright$ \sl #1}\medskip\nobreak}
\def\brf{\hangindent .4cm\hangafter 1}
\def\erf{\par\rm}
\def\ref#1#2#3#4#5{\brf\rmten #1 #2 {\bften #3 }({\rmten #4}) #5.\erf}
\def\cond{\leaders\hbox to 10pt{\hfil .\hfil}\hfill}
\def\ssc#1]{\noindent $\triangleright$ \sl #1}
% macros diverses
\def\SL{{\rm SL}(2,{\Bbb Z})}
\def\leff{L_{\rm eff}}\def\seff{S_{\rm eff}}
\def\sign{\mathop{\rm sign}\nolimits}
%
%macros pour la table des matieres
%
\def\cham#1#2{\medskip\bigskip\line{{\sectionfonte #1}\cond\nume #2}\bigskip}
\def\secm#1#2{\medskip\line{\kern 20pt {\bf #1}\cond\nume #2}\medskip}
\def\ssecm#1{\line{\kern 45pt $\triangleright$ \sl #1\hfill}}

